Knodle: Modular Weakly Supervised Learning with PyTorch

Strategies for improving the training and prediction quality of weakly supervised machine learning models vary in how much they are tailored to a specific task or integrated with a specific model architecture. In this work, we introduce Knodle, a software framework that treats weak data annotations, deep learning models, and methods for improving weakly supervised training as separate, modular components. This modularization gives the training process access to fine-grained information such as data set characteristics, matches of heuristic rules, or elements of the deep learning model ultimately used for prediction. Hence, our framework can encompass a wide range of training methods for improving weak supervision, ranging from methods that only look at correlations of rules and output classes (independently of the machine learning model trained with the resulting labels), to those that harness the interplay of neural networks and weakly labeled data. We illustrate the benchmarking potential of the framework with a performance comparison of several reference implementations on a selection of datasets that are already available in Knodle. The framework is published as an open-source Python package knodle and available at https://github.com/knodle/knodle.

==> chapters/old_vers/2_related_work_old.tex <==
\section{Related work}
\label{sec:related_work}

The high cost of manual expert annotation forces to find other methods of obtaining more labeled data with a lower effort.
One of them is \textit{active learning}, where only the automatically selected most valuable part of the data is manually annotated by experts \citep{Sun_2012}.
\textit{Semi-supervised learning} is used in cases when a small amount of data labeled by experts, but not enough itself to train a good model.
It is also often applied in the form of self-training models, that are iteratively trained using the labeled data and applied on unlabeled data in order to get the new annotated samples and incorporate them to training set \citep{kozareva-etal-2008-semantic,Agichtein_2000}.
However, the most relevant approach of overcoming the data bottleneck for our research is \textit{weak supervision}.
Its main idea is to annotate the dataset with potentially noisy labels with considerably reduced effort without using any manual expert annotation.
The weak supervision can be realised in different ways: by obtaining higher-level labels (for example, with some heuristic rules or high-level constraints \citep{Zhang_2017}) or lower-quality labels (obtained at a relatively small price, for example, by crowdsourcing \citep{Su_2018}).

\textbf{Distant Supervision.}

One of the most popular strategies of weak supervision is distant supervision, which is broadly used for relation extraction task.
It implies using of the knowledge from some existing sources and knowledge databases to annotate the unlabeled data.
Firstly the idea of distant supervision came about in \citep{Snow_2004} for automatically learning of \textit{is-a} \textit{(hypernym)} relations from text exploiting \textit{WordNet}.
Later, the other data sources, such as Wikipedia \citep{Wu_2007}, Freebase \citep{mintz-etal-2009-distant}, were proved to be effective for this task.

However, distant supervision inevitably produces different types of noise.
For example, distantly supervised data sometimes suffers from \textbf{incomplete labels} problem due to the incompleteness of knowledge bases used for distant supervision, what results in increasing the number of \textit{false negative} samples and in a lower recall.
Among the most popular approaches to mitigate the impact of incomplete labels is enhancing the knowledge base with the most likely relevant entries \citep{xu-etal-2013-filling}, more thorough construction of negative examples to balance the positive examples \citep{riedel-etal-2013-relation} and explicitly modelling of missing knowledge base information with latent variables \citep{Ritter_2013}.
Another problem of distant supervision is \textbf{noisy features} - increased amount of \textit{false positive} labels because of overgeneralised information from databases.
One of the most common approaches to solving this issue is considering relation extraction as a multi-instance problem.
Instead of (quite strong) original distant supervision assumption, a relaxed distant supervision assumption is used, which is formulated as the discriminative \textit{at-least-one} approach: there is at least one sentence in a dataset, that contains an entity pair and expresses the relation these entities are bound by in a knowledge base \citep{Riedel_2010}.
The relation variables are hidden in training, since it remains unknown, in how many sentences (but definitely in one or more) and in which sentence or sentences the relation is expressed.
Later, it was also extended to multi-instance multi-label learning problem \citep{hoffmann-etal-2011-knowledge,zeng-etal-2015-distant}.
Another solution to this problem is using topic models methods, such as generative probabilistic models \citep{yao-etal-2011-structured}, hierarchical topic models \citep{Roth_1013}, as well as their combination with the at-least-one approach \citep{Roth_2014}.
Sometimes the features denoising is provided in active learning manner with additional manual expertise \citep{Sterckx2014UsingAL}.
All of these approaches also differ according to the way the potentially noisy samples are treated: kept for further training with reduced weights \citep{jat2018improving,He_2020}, corrected \citep{shang2019noisy} or eliminated \citep{qin-etal-2018-robust}.

\textbf{Crowdsourcing Annotation.}
Another popular strategy of getting weakly annotated data is crowdsourcing - labeling the data by people who are not experts in the field and who can do annotation for much less money or even for free at some crowdsourcing platforms (for example, Amazon's Mechanical Turk (AMT)\footnote{https://www.mturk.com}).
This approach has already proven to be very successful on a great variety of natural language tasks, such as attribute extraction \citep{Su_2018}, word relations annotating \citep{Ahn_2006}, word similarity task, recognising textual entailment task and event annotation \citep{snow-etal-2008-cheap}.
As it was shown in \citep{snow-etal-2008-cheap}, not more than four non-expert contributors are necessary and sufficient in order to obtain a result which would be comparable with the one obtained from an expert.

However, the bottleneck of inaccurate supervision is the reliability of different annotators since their accuracy remains unknown.
The most trivial approach to detect the annotators’ errors is increasing of the workers number in order to get a set of several annotations of one dataset made by different annotators.
The correct annotation is chosen either with inter-annotator agreement measuring \citep{tratz2010taxonomy,Artstein_2018} or with majority voting \citep{Kosinski_2012}.
For denoising of errors produced by \textit{spammers}, who either randomly or by some strategy choose answers in order to maximise their payment, are used anomaly detection \citep{eskin-2000-detecting}, annotator's reliability modelling \citep{Dawid_1979}, bayseian approaches \citep{Vikas_2012} and generative models \citep{hovy-etal-2013-learning}.
The mistakes of careful but biased people (for example, parents with young children who tend to be more conservative and critical regarding the websites’ age requirement) could be easily predicted and, therefore, easily corrected, or “reversed” \citep{Ipeirotis_2010}.

The difference between distant supervision and crowdsourcing annotation methods is not as crucial as it might appear at the first glance.
We claim that the rules, or labeling functions, extracted from the knowledge base and used for distant supervision, could be regarded as the human annotators, since the label of the sample is decided basing them.
That means that the same principles and algorithms, including denoising methods, can be transferred to distantly supervised data and combined with each other.

\textbf{Structure learning.}
The goal of this line of research is to estimate the structure within a number of labeling functions.
While this is a much bigger field, we refer to structure learning within the weak supervision context. The intuition is that there is often some sort of correlation in between labeling functions.
It was first introduced by \citep{snorkel}.
Simultaneously the data programming paradigm was introduced which eases the generation of weakly labeled data sources.
Subsequently, improvements were made by \citep{DBLP:journals/corr/BachHRR17} or \citep{varma2019learning}.  \citep{DBLP:journals/corr/abs-1911-09860} made improvements by using stochastic, or more specifically, quality guided labeling functions. An extension to semi-supervision was made by \citep{maheshwari2020data}.
%In addition, various applications were introduced, including
% biology
% what about subset paper?

\textbf{Noise-aware learning.} A prominent idea is to use a architecture which accounts for noisy data.  The research branch is relevant because weak labels can be seen as very noisy labels. 
Many try to model noise-robustness by adapting the loss function.
\citep{patrini2017making} perform a noise adaption after the loss calculation.  In \citep{zhang2018generalized} a generalization of cross-entropy and the mean absolute error is introduced.
Alternatively, in \citep{sukhbaatar2015training} the authors add a noise layer in a convolutional neural network.
Many approaches are based on noise assumptions. For instance \citep{vanrooyen2015learning} make the assumption of symmetric label noise.
Another approach aims at finding and removing wrongly labeled samples from the training procedure.
Recently, the confidence learning framework Cleanlab was introduced in \citep{northcutt2021confident}.
It is based on the intuition, that low-confidence predictions are more likely to be labeled wrongly.

\textbf{Frameworks.}
Knodle builds up upon on the ideas of several software frameworks.
On a low level,  Knodle is built on top of PyTorch, \citep{NEURIPS2019_9015}.
We took design decisions from several other high level libraries which aim to ease the training and prediction experience.
Namely,  we drew inspiration from PyTorch lightning by \citep{falcon2019pytorch} which in essence tries to remove the burdance of writing your own train loop and Huggingface's Transformers library, \citep{wolf2020huggingfaces} which gives easy access to various transformer-based architectures.
Particularly, we took over the Trainer class design both use.
Finally, we look at the Snorkel framework by \citep{snorkel}. It provides functionality to work with labeling functions and to train a structure learning model.
It's very easy to use Snorkel to prepare data suitable for Knodle.




==> chapters/old_vers/3_model_andy.tex <==
\section{Weakly supervised learning with knodle}

\subsection{Formal description}

Knodle provide a new layer of abstractions that allows the integration of weakly supervised learning signals and denoising algorithms into PyTorch.
The framework follows two design principles, outlined below.
\\
\\
The \textbf{first design principle} is that knodle is driven by tensor-based representations of input data and weak labels.
Similar to Pytorch, where the data is already assumed to be in Tensor form, and the specific choices of pre-processing that led to a particular input representation are outside the scope of the core deep learning model, we choose to exclude the process of heuristic labeling from the knodle framework.
We represent the weak labels in a two-step process.
Note that we often use the terms weak label, labeling function or rule interchangeably.
From now on we assume $r$ rules and $k$ classes.
Rule matches are gathered in a binary matrix $Z \in \lbrace 0, 1 \rbrace^{n \times r}$, $Z_{ij}=1$ if rule $j$ matches sample $i$, and the initial mapping from rules to the corresponding classes is given by another binary matrix $T \in \lbrace 0, 1 \rbrace^{r \times k}$, $T_{jk}=1$ if rule $j$ is indicative of class $k$.
\\
\\
The \textbf{second design principle} is the separation between the prediction model from the weak supervision aspects of the training.
Therefore the same model definition can be used for training based on direct or weak supervision, allowing to easily create benchmark setups.
However, even though the the prediction model is defined separately from the denoising algorithm, the denoising algorithm has access to the model class during training.
%Difference description:
Denoising and model training can hence reinforce each other in an integrated manner.
For example, cross-validation schemes (see Section XX) can use the model architecture to reweight instances during training.
This is in contrast to approaches that modularize denoising and training by first adjusting label confidences looking at label function correlations only and then training a model using the adjusted labels (Takamatsu, Snorkel).
The knodle design is also in contrast to approaches where denoising is so integrated into the model already that it cannot be separated as an independent principle and generally applied to other deep learning models that map inputs to outputs.
\\
\\
Formally, the knodle software framework will learn the parameters for a neural classification network $f: \reals^{f} \rightarrow \reals^{k}$.
Importantly, it does \textbf{not} directly rely on the weak labels $\hat{Y}$.
Instead, it will consider on a model, $X$, $Z$ and $T$ to achieve the best possible generalization, according to one of the algorithms that are provided within the framework.

\subsection{Denoising algorithms implemented in knodle}
\label{subsec:model_impl}

To ensure a seamless use of the developed algorithms, the weakly supervised algorithms need to be tightly integrated with automatic differentiation and optimization supported by PyTorch.
For example, in rule-adversarial learning, a second prediction layer for the adversarial objective (that aims at identifying matching rules) needs to be added to the model automatically, and the gradients stemming from the adversarial objective need to be reversed appropriately.

All of this is done within \texttt{Trainer} classes.
During initialization, they receive data, a model, possibly pre-initialized or pretrained, and a method specific configuration, inheriting from \texttt{Config}.
The following example call, illustrates the usage of the rule-adversarial method \textit{WSCrossWeigh}, which we describe below:%
\\
\\
\centerline{\texttt{CrossWeighTrainer(model, X, Z, T, config).train()}}
\\
\\
We already provide some out-of-the-box trainers which can serve as baselines or starting point for further investigations.
Currently, the Trainers are able to use all models that expect a list of tensor as input;
Knodle provides logistic regression and HuggingFace's \texttt{transformers} \citep{wolf2020huggingfaces} classification models as an example.

\textbf{Majority Voting Baseline.}
In order to get an impression, how good labeling functions are, a simple majority voting is used as a baseline.
As was already mentioned in Section \ref{sec:related_work}, it is one of the most basic approaches to denoising the data labeled by two or more labeling functions or human annotators.
In \knodle{} it is realised as follows: the test dataset is, firstly, annotated with the labeling functions, and then labels got in such way are compared with the gold ones, known for this dataset.

\textbf{Trainer without Denoising.}
The simplest model is the \texttt{NoDenoisingTrainer}.
The majority vote is computed and used to train the given model.
This is the easiest baseline, we could think of, as it consists only of a format change from $Z, T$ to $Y$ and a standard training loop.
Throughout this work, majority vote takes the maximum number of matching rules or samples uniformly from the best choices, if no clear majority exists. 
It can either be a single label or a probabilistic label.

\textbf{kNN Denoising Method.}
Secondly, we implemented the \texttt{KNNDenoisingTrainer}.
We want to provide a simple label denoising trainer with a simple geometric interpretation.
The intuition behind this method is that similar samples should be activated by the same rules.
Thus, we make a smoothness assumption on the target space.
The trainer looks at the $k$ most similar samples, for example, by tfidf features combined with $L_2$ distance, and activates the rules matching the neighbors to create a denoised $\hat{Z}$.
We allow separate features for the model training and the neighborhood activation.
Note that this method provides a way to activate rules for unmatched samples.

\textbf{Snorkel Denoising Method.}
Additionally, we provide a wrapper of the Snorkel system, \mbox{\texttt{SnorkelTrainer}}.
By doing so, the show how easy it is to incorporate existing systems into knodle.
Our trainer incorporates both Snorkel steps, the generative and discriminative step.
First, Snorkel aims to learn the structure within labels and rules, in our notation $P(Y, Z, T)$ in an unsupervised fashion.
The authors call this the generative model.
Afterwards the training of the final discrimative model, approximating $P(Y|X)$ according to the labels provided by the generative model is computed.
We provide a mix of the latter two, called \texttt{SnorkelKNNDenoisingTrainer}, which was easily implemented in a few lines of code, using the
of knodle.

\textbf{Distant Supervision CrossWeigh Denoising Method.}
The Distant Supervision CrossWeigh is an algorithm for noise correction in distantly annotated data based on the CrossWeight Framework in \citep{wang-etal-2019-crossweigh} proposed for mistakes identification in crowdworkers annotations.
The main denoising idea is to detect the sentences, which are annotated with potentially wrong labels, and reduce their importance for final classifier training.

Though the original CrossWeigh Framework was proposed for mistakes identification in crowdworkers annotations, we claim that it could be also applied for denoising the distantly supervised data.
Indeed, the decision rules in distant supervision could be regarded as human annotators, since the label of the sample is decided basing them.
Thus, if the same decision rule is annotated with a wrong label over the training set, the model is likely to learn the wrong pattern and to make similar mistakes while labeling the test samples.
However, if we take a sufficiently big data \textit{without} samples with this particular decision rule (that is, without samples containing this particular mistake in their annotation), train the model on it and then classify the test samples, the predictions are supposed to contradict the initial \textit{wrong} labels.

The first part of the algorithm aims at detecting in weakly annotated training set \textit{$\textbf{D} = [\{x_1, ..., x_{m}\}, \{y_1, ..., y_{m}\}]$} the sentences, which are annotated with potentially wrong labels.
As in the original CrossWeigh Framework, the basic idea is similar to the \textit{k}-fold cross validation, where input data is splitted into \textit{k} folds, each of which becomes in turn a test set, while the model is trained on the others and tested on the hold-out fold.

The splitting is performed basing on labeling functions.
Thus, firstly, the labeling functions are randomly splitted into \textbf{\textit{K}} folds $\{r_1, ..., r_k\}$ and, iteratively, each fold $fold_l$ is chosen to form a test set, which is build from all samples matched this fold's labeling functions.
Other samples, on their turn, build a training set in order to train a classifier on it.
The trained model is tested on hold-out fold samples.
The predicted label $\hat{y_i}$ for each test sample $x_i$ is then compared to the label $y_i$ originally assigned to $x_i$ by distant supervision.
If $\hat{y_i} \neq{y_i}$, the sample $x_i$ is claimed to be potentially mislabeled and its \textit{confidence coefficient} - a parameter which is assigned to a sentence $x_i$ to reflect how confident the system is that $x_i$ is wrongly labeled - is increased by one.

The mistake estimation module is repeated several times.
After all rounds are done, the confidence coefficient $c_i$ for each sample $x_i$ is turned to sample weight $w_{x_i}$ using an empirically estimated parameter $\epsilon$: \[w_i = \epsilon^{c_i}\]
Thus, the more probable the original $y_i$ label of data sample $x_i$ is wrong, the smaller weight $w_{x_i}$ the dataset gets, and, therefore, the smaller part it will play in further training.
When the sample weights are calculated, the final classifier is trained on the whole reweighed dataset.



==> chapters/old_vers/3_model_ben.tex <==
\section{Weakly supervised learning with Knodle}

% Check out actual usage
%% Pytorch
%% Knodle

% Settings can also be characterized by following high-level choices:
%% generating negative instances
%% special labels like no_rel
%% additional unsupervised data
%% general or binary Cross-Entropy 

The standard setting for supervised machine learning is to learn a mapping from input tensor(s) to output tensor(s) guided by a loss function that measures the faithfulness of the learned mapping to the observed output values.
Deep learning frameworks like PyTorch support learning in this regime, and input tensors, output tensors, as well as the loss function are modularized and are provided to the learning mechanism as isolated objects, e.g., as method arguments.

In the simplest setting, training data for multi-class classification is represented by a \emph{design matrix} $X \in \mathbb{R}^{n \times f}$ ($n$ instances represented by $f$ features/input dimensions) and a \emph{label matrix} $Y \in \mathbb{R}^{n \times k}$ ($k$ classes). When the model details have been specified, training can be executed by simple high-level call, e.g.:\\
\centerline{\texttt{model.train(X,Y)}}

Deep learning frameworks, such as TensorFlow \citep{Abadi2016TensorFlowAS} and PyTorch \cite {Paszke2017AutomaticDIPytorch}, hide modeling and optimization details by suitable layers of abstractions.

%The recent success of neural networks in almost all areas of machine learning is to a large degree due to the development of modular software architectures that package arbitrarily complex models into astonishingly simple abstractions.

Knodle's goal is to provide a new layer of abstractions that allows the integration of weakly supervised learning signals and denoising algorithms into PyTorch.
The \textbf{first design principle} is that Knodle is driven by tensor-based representations of input data and labeling function matches.
Similar to Pytorch, where the data is already assumed to be in Tensor form, and the specific choices of pre-processing that led to a particular input representation are outside the scope of the core deep learning model, we choose to not make the process of heuristic labeling a part of the Knodle framework.
Rather, we encode all the essential information about the weak labeling process in tensors, namely one tensor that contains information about which labeling functions matched for each data instance, and another tensor describing the relationship between labeling functions and output classes.
All the procedural details that led to matches of the labeling functions, i.e. the original input data, patterns, etc., are not part of the type of process that can be modeled with Knodle.

Specifically, in weakly supervised learning, (heuristic) labels are obtained in a two-step process:
Rule matches can be gathered in a binary matrix $Z \in \reals^{n \times r}$ ($r$ rules, $Z_{ij}=1$ iff rule $j$ matches for sample $i$), and the initial mapping from rules to the corresponding classes of interest can be given by another binary matrix $T \in \reals^{r \times k}$ ($T_{jk}$ iff rule $j$ is indicative for class $k$).
Traditional weak-supervision approaches would then use a (suitably normalized) noisy heuristic label matrix $Y_{heur} =ZT$ for training, entailing all problems of naive weak supervision, such as false positives and false negatives.

The \textbf{second design principle} is that weakly supervised training separates the prediction model (a classical Pytorch deep learning model for mapping inputs to output classes) from the weak supervision aspects of the training (including denoising and generalization from labeling functions). I.e. the same model definition can be used for training based on direct or weak supervision. 
However, even though the the prediction model is defined seperately from the denoising algorithm, the denoising algorithm has access to the model class during training. 
Denoising and model training can hence reinforce each other in an integrated manner. 
For example, cross-validation schemes (see Section XX) can use the model architecture to reweight instances during training. 
This is in contrast to approaches that modularize denoising and training by first adjusting label confidences looking at label function correlations only and then training a model using the adjusted labels (Takamatsu, Snorkel).
The Knodle design is also in contrast to approaches where denoising is so integrated into the model already that it cannot be separated as an independent principle and generally applied to other deep learning models that map inputs to outputs.

Formally, the Knodle software framework will learn the parameters for a neural classification network ($\reals^{f} \rightarrow \reals^{k}$), but it would \textbf{not} rely on $Y_{heur}$. 
Instead, it will consider $X$, $Z$ and $T$ to achieve the best possible generalization, according to one of the algorithms for weakly supervised algorithms that are provided within the framework.
That is, the highest level of abstraction will allow for a training call similar to the following (with the option to specify the type of denoising algorithm, e.g., rule-adversarial learning):\\
\centerline{\texttt{model.train(X,Z,T, denoising='cross-weight')}}

For enabling such a seamless use of the developed algorithms, while keeping the already existing modularity of the deep learning frameworks intact,
the weakly supervised algorithms need to be tightly integrated with automatic differentiation and optimization supported by PyTorch.
For example, in rule-adversarial learning, a second prediction layer for the adversarial objective (that aims at identifying matching rules) needs to be added to the model automatically, and the gradients stemming from the adversarial objective need to be reversed appropriately. 
The joint architecture thus constitutes a classifier with an integrated adversarial component. 
Other methods (such as those based on outlier detection), would aim at estimating better versions of $Y_{heur}$ together with sample weights repeatedly for each training batch.

==> chapters/old_vers/4_methods.tex <==
%\section{Methods}
%
%\subsection{Distant Supervision CrossWeigh Framework (WSCrossWeigh)}

%The Distant Supervision CrossWeigh is an algorithm for noise correction in distantly annotated data based on the CrossWeight Framework in \citep{wang-etal-2019-crossweigh} proposed for mistakes identification in crowdworkers annotations.
%The main denoising idea is to detect the sentences, which are annotated with potentially wrong labels, and reduce their importance for final classifier training.
%
%Though the original CrossWeigh Framework was proposed for mistakes identification in crowdworkers annotations, we claim that it could be also applied for denoising the distantly supervised data.
%Indeed, the decision rules in distant supervision could be regarded as human annotators, since the label of the sample is decided basing them.
%Thus, if the same decision rule is annotated with a wrong label over the training set, the model is likely to learn the wrong pattern and to make similar mistakes while labeling the test samples.
%However, if we take a sufficiently big data \textit{without} samples with this particular decision rule (that is, without samples containing this particular mistake in their annotation), train the model on it and then classify the test samples, the predictions are supposed to contradict the initial \textit{wrong} labels.
%
%Let us introduce the notation first.
%
%
%The first part of the algorithm aims at detecting in weakly annotated training set \textit{$\textbf{D} = [\{x_1, ..., x_{m}\}, \{y_1, ..., y_{m}\}]$} the sentences, which are annotated with potentially wrong labels.
%As in the original CrossWeigh Framework, the basic idea is similar to the \textit{k}-fold cross validation, where input data is splitted into \textit{k} folds, each of which becomes in turn a test set, while the model is trained on the others and tested on the hold-out fold.
%
%The splitting is performed basing on labeling functions.
%Thus, firstly, the labeling functions are randomly splitted into \textbf{\textit{K}} folds $\{r_1, ..., r_k\}$ and, iteratively, each fold $fold_l$ is chosen to form a test set, which is build from all samples matched this fold's labeling functions.
%Other samples, on their turn, build a training set in order to train a classifier on it.
%The trained model is tested on hold-out fold samples.
%The predicted label $\hat{y_i}$ for each test sample $x_i$ is then compared to the label $y_i$ originally assigned to $x_i$ by distant supervision.
%If $\hat{y_i} \neq{y_i}$, the sample $x_i$ is claimed to be potentially mislabeled and its \textbf{\textit{confidence coefficient}} - a parameter which is assigned to a sentence $x_i$ to reflect how confident the system is that $x_i$ is wrongly labeled - is increased by one.
%
%The mistake estimation module is repeated \textbf{\textit{R}} CrossWeigh rounds.
%After all rounds are done, the confidence coefficient $c_i$ for each sample $x_i$ is turned to sample weight $w_{x_i}$ using an empirically estimated parameter $\epsilon$: \[w_i = \epsilon^{c_i}\]
%Thus, the more probable the original $y_i$ label of data sample $x_i$ is wrong, the smaller weight $w_{x_i}$ the dataset gets, and, therefore, the smaller part it will play in further training.
%When the sample weights are calculated, the final classifier is trained on the whole reweighed dataset.






%\textbf{Discuss:}
%
%\begin{itemize}
%    \item Where to introduce z and t properly?
%    My suggestion: In here
%\end{itemize}

==> chapters/old_vers/6_discussion.tex <==
\section{Discussion of Data Model}

First, we compare our tensor.based data abstraction to 

\textbf{Snorkel.} There exist other ways to represent $Z$ and $T$.
Here, we want to compare with the probably most common alternative which is introduced by the Snorkel framework \citep{snorkel}
A single label matrix $\Lambda \in \lbrace-1,  0, \dots,  c \rbrace^{n \times m}$ is used,  where $\Lambda_{i, j}=k$ denotes that rule $j$ assigned class $k \in [c]$ to sample $i$,.  Note that $-1$ refers to abstaining. 
Mathematically,  one can easily construct a bijection.  Practically,  $\Lambda$ provides a single dense data structure whereas $Z$ and $T$ benefit from sparsification.
this proved helpful for lager scenarios such as IMDb or Tacred.
\\
\\
\textbf{Extensions.} Additionally,  one might think of an confidence score of a weak label, as in \citep{DBLP:journals/corr/abs-1911-09860}.
By relaxing individual rules $Z_{ij} \in [0, 1]$ or all rules $T_{ij} \in [0, 1]$,  it's easy to encode additional information.
Moreover, we can easily extend the input to multi-task learning by transforming the $T$ matrix to a tensor $T \in \lbrace 0, 1 \rbrace^{m \times t \times c^*}$, where $t$ is number of tasks and $c^*=\max_t c_t$. 
From an applied point of view, we are pleased to see that the current implementation only needs minimal modifications to enable these extensions.

==> iclr_format/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

